Efficient space-time reduced order model for linear dynamical systems in Python using less than 120 lines of code

A classical reduced order model (ROM) for dynamical problems typically involves only the spatial reduction of a given problem. Recently, a novel space-time ROM for linear dynamical problems has been developed, which further reduces the problem size by introducing a temporal reduction in addition to a spatial reduction without much loss in accuracy. The authors show an order of a thousand speed-up with a relative error of less than 0.00001 for a large-scale Boltzmann transport problem. In this work, we present for the first time the derivation of the space-time Petrov-Galerkin projection for linear dynamical systems and its corresponding block structures. Utilizing these block structures, we demonstrate the ease of construction of the space-time ROM method with two model problems: 2D diffusion and 2D convection diffusion, with and without a linear source term. For each problem, we demonstrate the entire process of generating the full order model (FOM) data, constructing the space-time ROM, and predicting the reduced-order solutions, all in less than 120 lines of Python code. We compare our Petrov-Galerkin method with the traditional Galerkin method and show that the space-time ROMs can achieve O(100) speed-ups with O(0.001) to O(0.0001) relative errors for these problems. Finally, we present an error analysis for the space-time Petrov-Galerkin projection and derive an error bound, which shows an improvement compared to traditional spatial Galerkin ROM methods.

==> commands.tex <==
\usepackage{enumitem}

\newlist{Assumption}{enumerate}{1}
\setlist[Assumption]{label=A\arabic*}

%\textbf{}%\renewcommand{\familydefault}{\sfdefault} 


\definecolor{Blue}{rgb}{0,0,1}
\definecolor{Red}{rgb}{1,0,0}
\definecolor{Green}{rgb}{0,1,0}
%\newcommand{\snaps}[1]{\ensuremath{\snapsNo_{#1}}}  % timestep at optional
\newcommand{\ZD}[1]{{\textcolor{Blue}{ZD: #1}}}
\newcommand{\YC}[1]{{\textcolor{Red}{YC: #1}}}
\newcommand{\fontContinuousFunc}{ }
\newcommand{\timevar}{t}
\newcommand{\statemat}{\boldsymbol{A}}
\newcommand{\inputmat}{\boldsymbol{B}}
\newcommand{\inputvec}{\boldsymbol{f}}
\newcommand{\initialstate}{\state_0}
\newcommand{\outputmat}{\boldsymbol{C}}
\newcommand{\outputvec}{\boldsymbol{y}}
\newcommand{\fontDiscreteFunc}{\mathscr}
\newcommand{\fontDiscrete}{\mathcal}
\newcommand{\fontSubspace}{\mathcal}
\newcommand{\knArg}[1]{k(t^{#1})}
\newcommand{\kn}{\knArg{n}}
\newcommand{\knDummy}{k(\timeDummy^n)}
\newcommand{\kmax}{k_\text{max}}
\newcommand{\bds}[1]{{\boldsymbol{#1}}}
\newcommand{\highlight}[1]{{\textcolor{Red}{#1}}}
\newcommand{\defeq}{:=}
\newcommand{\eqdef}{=:}
\newcommand{\SPSD}[1]{\text{SPSD}(#1)}
\newcommand{\optDummy}{v}
\newcommand{\orthomat}[2]{\mathbb V_{{#2}}(\RR{{#1}})}
\newcommand{\domain}{\Omega}
\newcommand{\domaini}{\domain_i}
\newcommand{\boundary}{\Gamma}
\newcommand{\mappingNo}{\mathcal I}
\newcommand{\mapping}[2]{\mappingNo(#1,#2)}
\newcommand{\boundaryi}{\boundary_i}
\newcommand{\nsubdomains}{{n_\domain}}
\newcommand{\nconstraints}{n_{\bar A}}
\newcommand{\nconstraintsROM}{n_{A}}
\newcommand{\ninterfacedofs}{{n_\boundary}}
\newcommand{\residual}{\bds{r}}
\newcommand{\residualArg}[1]{\residual_{#1}}
\newcommand{\residuali}{\residualArg{i}}
\newcommand{\methodAcronym}{ST-LSPG}
\newcommand{\timeSpace}{\fontContinuousFunc H}
\newcommand{\timeDiscreteFuncSpace}{\fontDiscreteFunc H}
\newcommand{\timeDiscreteSpace}{\RR{\ntimedof}}
\newcommand{\spatialSpace}{\RR{\nspacedof}}
\newcommand{\unrollfuncNo}{\bds{g}}
\newcommand{\unrollfunc}[1]{{\unrollfuncNo}(#1)}
\newcommand{\unrollNone}{\unrollfuncNo} % timestep at optional
\newcommand{\vectorizeNone}{\vectorizefuncNo} % timestep at optional
\newcommand{\vectorize}[1]{\ensuremath{\vectorizeNone(#1)}}  % timestep
\newcommand{\vectorizeinv}[1]{\ensuremath{\vectorizeNone^{-1}(#1)}}  %
\newcommand{\vectorizefuncNo}{\bds{h}}
\newcommand{\vectorizefunc}[1]{{\vectorizefuncNo}(#1)}
\newcommand{\lipschitzK}{L_{\res}}
\newcommand{\inverseLipschitzK}{K_{\res}}
\newcommand{\lipschitzFK}{L_{\flux}}
\newcommand{\inverseLipschitzFK}{K_{\flux}}
\newcommand{\boundingConstantF}{M_{\flux}}
\newcommand{\arbitraryConstant}{C}
\newcommand{\bignum}{N}
\newcommand{\smallnum}{n}
\newcommand{\abarConstant}{\kappa_1}
\newcommand{\aConstant}{\kappa_2}


\newcommand{\stateContinuousDummyEntryNo}{\boldsymbol{u}}
\newcommand{\stateContinuousDummyEntry}[1]{\stateContinuousDummyEntryNo_{#1}}
\newcommand{\stateContinuousDummy}[1]{\bds{\stateContinuousDummyEntryNo}} 
\newcommand{\stateTwoContinuousDummyEntryNo}{\boldsymbol{v}}
\newcommand{\stateTwoContinuousDummyEntry}[1]{\stateTwoContinuousDummyEntryNo_{#1}}
\newcommand{\stateTwoContinuousDummy}[1]{\bds{\stateTwoContinuousDummyEntryNo}} 
\newcommand{\metric}{\bds{\Theta}} 

\newcommand{\crossareaSymb}{A}
\newcommand{\externalforceSymb}{q}
\newcommand{\externalforce}{\boldsymbol \externalforceSymb}
\newcommand{\state}{\bds{x}}
\newcommand{\stateArg}[1]{\state^{#1}}
\newcommand{\statei}{\stateArg{i}}

\newcommand{\stateApprox}{\tilde\state}
\newcommand{\stateApproxArg}[1]{\stateApprox_{#1}}
\newcommand{\stateApproxi}{\stateApproxArg{i}}
\newcommand{\stateApproxInterior}{\tilde\state^\domain}
\newcommand{\stateApproxInteriorArg}[1]{\stateApproxInterior_{#1}}
\newcommand{\stateApproxInteriori}{\stateApproxInteriorArg{i}}
\newcommand{\stateApproxBoundary}{\tilde\state^\boundary}
\newcommand{\stateApproxBoundaryArg}[1]{\stateApproxBoundary_{#1}}
\newcommand{\stateApproxBoundaryi}{\stateApproxBoundaryArg{i}}

\newcommand{\stateInterior}{\bds{x}^{\Omega}}
\newcommand{\stateInteriorArg}[1]{\stateInterior_{#1}}
\newcommand{\stateInteriori}{\stateInteriorArg{i}}

\newcommand{\stateBoundary}{\bds{x}^{\Gamma}}
\newcommand{\stateBoundaryArg}[1]{\stateBoundary_{#1}}
\newcommand{\stateBoundaryi}{\stateBoundaryArg{i}}

\newcommand{\projection}{\bds{P}}
\newcommand{\projectionRes}{\projection^\residual}
\newcommand{\projectionResArg}[1]{\projectionRes_{#1}}
\newcommand{\projectionResi}{\projectionResArg{i}}

\newcommand{\projectionStateInterior}{\projection^\Omega}
\newcommand{\projectionStateInteriorArg}[1]{\projectionStateInterior_{#1}}
\newcommand{\projectionStateInteriori}{\projectionStateInteriorArg{i}}

\newcommand{\projectionStateBoundary}{\bds{P}^\Gamma}
\newcommand{\projectionStateBoundaryArg}[1]{\projectionStateBoundary_{#1}}
\newcommand{\projectionStateBoundaryi}{\projectionStateBoundaryArg{i}}


\newcommand{\rbGlobal}{\bds{\Phi}}
\newcommand{\rbBubble}{\bds{\Phi}^\domain}
\newcommand{\rbBubbleArg}[1]{\rbBubble_{#1}}
\newcommand{\rbBubblei}{\rbBubbleArg{i}}
\newcommand{\rbBoundary}{\bds{\Phi}^\boundary}
\newcommand{\rbBoundaryArg}[1]{\rbBoundary_{#1}}
\newcommand{\rbBoundaryi}{\rbBoundaryArg{i}}
\newcommand{\rbInterior}{\bds{\Phi}^\domain}
\newcommand{\rbInteriorArg}[1]{\rbInterior_{#1}}
\newcommand{\rbInteriori}{\rbInteriorArg{i}}
\newcommand{\rbPort}{\bds{\Phi}^p}
\newcommand{\rbPortArg}[1]{\rbPort_{#1}}
\newcommand{\rbPorti}{\rbPortArg{i}}
\newcommand{\rbPortj}{\rbPortArg{j}}
\newcommand{\rbInterface}{\bds{\Phi}^y}

\newcommand{\redState}{\hat {\bds x}}
\newcommand{\redStateArg}[1]{\redState_{#1}}
\newcommand{\redStateBoundary}{\redState^\boundary}
\newcommand{\redStateBoundaryArg}[1]{\redStateBoundary_{#1}}
\newcommand{\redStateBoundaryi}{\redStateBoundaryArg{i}}
\newcommand{\redStateBoundaryisol}{\redStateBoundaryArg{i\star}}
\newcommand{\redStateBoundaryNullVar}{\bds{y}}
\newcommand{\redStateBoundaryNull}{\redStateBoundaryNullVar^\boundary}

\newcommand{\redStateInterface}{\hat{\bds{y}}}

\newcommand{\redStateInterior}{\redState^\domain}
\newcommand{\redStateInteriorArg}[1]{\redStateInterior_{#1}}
\newcommand{\redStateInteriori}{\redStateInteriorArg{i}}
\newcommand{\redStateInteriorisol}{\redStateInteriorArg{i\star}}


%dimensions
\newcommand{\ndof}{\nspacedof}
\newcommand{\ndofi}{n_i}
\newcommand{\ndofInteriori}{n^{\Omega}_i}
\newcommand{\ndofBoundaryi}{n^{\Gamma}_i}
\newcommand{\nresi}{n^\residual_i}
\newcommand{\weightmatRows}{z}
\newcommand{\weightmatRowsArg}[1]{\weightmatRows^{#1}}
\newcommand{\weightmatRowsn}{\weightmatRowsArg{n}}
\newcommand{\weightmatstRows}{\bar z}
\newcommand{\weightmatstRowsArg}[1]{\weightmatstRows^{#1}}
\newcommand{\weightmatstRowsn}{\weightmatstRowsArg{n}}

\newcommand{\nrb}{p}
\newcommand{\nrbInterior}{\nrb^\domain}
\newcommand{\nrbInteriorArg}[1]{\nrbInterior_{#1}}
\newcommand{\nrbInteriori}{\nrbInteriorArg{i}}
\newcommand{\nrbBoundary}{\nrb^\boundary}
\newcommand{\nrbBoundaryArg}[1]{\nrbBoundary_{#1}}
\newcommand{\nrbBoundaryi}{\nrbBoundaryArg{i}}
\newcommand{\nrbPort}{\nrb^p}
\newcommand{\nrbPortArg}[1]{\nrbPort_{#1}}
\newcommand{\nrbPorti}{\nrbPortArg{i}}
\newcommand{\nrbPortj}{\nrbPortArg{j}}
\newcommand{\nrbInterface}{\nrb^y}


\newcommand{\constraintMat}{\bds{\bar A}}
\newcommand{\constraintMatArg}[1]{\constraintMat_{#1}}
\newcommand{\constraintMati}{\constraintMatArg{i}}
\newcommand{\constraintMatROM}{\bds{A}}
\newcommand{\constraintMatROMArg}[1]{\constraintMatROM_{#1}}
\newcommand{\constraintMatROMi}{\constraintMatROMArg{i}}

\newcommand{\hessianIntInt}{\bds{H}^{\domain\domain}}
\newcommand{\hessianIntIntArg}[1]{\hessianIntInt_{#1}}
\newcommand{\hessianIntInti}{\hessianIntIntArg{i}}


\newcommand{\hessianIntBound}{\bds{H}^{\domain\boundary}}
\newcommand{\hessianIntBoundArg}[1]{\hessianIntBound_{#1}}
\newcommand{\hessianIntBoundi}{\hessianIntBoundArg{i}}

\newcommand{\hessianBoundInt}{\bds{H}^{\boundary\domain}}
\newcommand{\hessianBoundIntArg}[1]{\hessianBoundInt_{#1}}
\newcommand{\hessianBoundInti}{\hessianBoundIntArg{i}}

\newcommand{\hessianBoundBound}{\bds{H}^{\boundary\boundary}}
\newcommand{\hessianBoundBoundArg}[1]{\hessianBoundBound_{#1}}
\newcommand{\hessianBoundBoundi}{\hessianBoundBoundArg{i}}

\newcommand{\searchDirInterior}{\bds{p}^\domain}
\newcommand{\searchDirInteriorArg}[1]{\searchDirInterior_{#1}}
\newcommand{\searchDirInteriori}{\searchDirInteriorArg{i}}

\newcommand{\searchDirLagrange}{\bds{p}^\lagrange}
\newcommand{\searchDirInterface}{\bds{p}^\redStateBoundaryNullVar}

\newcommand{\searchDirBoundary}{\bds{p}^\boundary}
\newcommand{\searchDirBoundaryArg}[1]{\searchDirBoundary_{#1}}
\newcommand{\searchDirBoundaryi}{\searchDirBoundaryArg{i}}

\newcommand{\redResState}{\hat{\bds{r}}_\bds{x}}
\newcommand{\redResLagrange}{\hat{\bds{r}}_\lagrange}

\newcommand{\redResBoundary}{\hat{\bds{r}}^\boundary}
\newcommand{\redResBoundaryArg}[1]{\redResBoundary_{#1}}
\newcommand{\redResBoundaryi}{\redResBoundaryArg{i}}

\newcommand{\redResInterior}{\hat{\bds{r}}^\domain}
\newcommand{\redResInteriorArg}[1]{\redResInterior_{#1}}
\newcommand{\redResInteriori}{\redResInteriorArg{i}}

\newcommand{\dualProblem}{h}
\newcommand{\dualProblemArg}[1]{\dualProblem_{#1}}
\newcommand{\dualProblemi}{\dualProblemArg{i}}

\newcommand{\unitvec}{\bds{e}}
\newcommand{\unitvecArg}[1]{\unitvec_{#1}}
\newcommand{\spacetimeindexNo}{\varphi}
\newcommand{\spacetimeindex}[2]{\varphi(#1,#2)}
\newcommand{\spacetimeindexIncludeAll}[1]{\spacetimeindex{\spaceindex{#1}}{\timeindex{#1}}}
\newcommand{\spacetimeindexIncludeAllSmall}[1]{\spacetimeindex{\spaceindexsmall{#1}}{\timeindexsmall{#1}}}
\newcommand{\spaceindexNo}{\mathcal s}
\newcommand{\timeindexNo}{\mathcal t}
\newcommand{\spaceindex}[1]{\mathcal s_{#1}}
\newcommand{\timeindex}[1]{\mathcal t_{#1}}
\newcommand{\spaceindexsmall}[1]{\mathcal s_{#1}'}
\newcommand{\timeindexsmall}[1]{\mathcal t_{#1}'}
\newcommand{\spacetimesampleset}{\mathfrak{st}}
\newcommand{\spacetimesamplesetsmall}{\spacetimesampleset'}
\newcommand{\samplematstsmall}{\samplematst'}

\newcommand{\resIndexSet}{I}
\newcommand{\resIndexSetArg}[1]{\resIndexSet_{#1}}
\newcommand{\resIndexSeti}{\resIndexSetArg{i}}

\newcommand{\nullspacemat}{\bds{B}}
\newcommand{\nullspacematArg}[1]{\nullspacemat_{#1}}
\newcommand{\nullspacemati}{\nullspacematArg{i}}

\newcommand{\redNullspacemat}{\hat{\bds{B}}}
\newcommand{\redNullspacematArg}[1]{\redNullspacemat_{#1}}
\newcommand{\redNullspacemati}{\redNullspacematArg{i}}

\newcommand{\identityi}{\bds{E}_i}
\newcommand{\uncoupledMiniNo}{g_i}
\newcommand{\uncoupledMini}[1]{\uncoupledMiniNo(#1)}
\newcommand{\lagrange}{\bds{\lambda}}
\newcommand{\lagrangian}{L}
\newcommand{\zero}{\bds{0}}
\newcommand{\argmin}[1]{\underset{#1}{\text{argmin}}}
\newcommand{\range}[1]{\text{range}(#1)}
\newcommand{\subdomainPorts}[1]{P(#1)}
\newcommand{\portsSubdomains}[1]{Q(#1)}
\newcommand{\portsSubdomainsTwo}[2]{Q(#1,#2)}
\newcommand{\nports}{{n_p}}
\newcommand{\nportsSub}[1]{{\nports(#1)}}
\newcommand{\ndofPorts}[1]{n^p}
\newcommand{\ndofPortsArg}[1]{n_{#1}^p}
\newcommand{\ndofPortsj}{\ndofPortsArg{j}}
\newcommand{\projectionStatePort}[2]{\projection^{#1}_{#2}}
\newcommand{\projectionStatePortAll}[1]{\projection^{#1}}
\newcommand{\nconstraintsPort}[1]{n^c_{#1}}
%\newcommand{\card}[1]{\text{card}(#1)}
\newcommand{\card}[1]{|#1|}
\newcommand{\RRstar}[1]{\mathbb{R}_\star^{#1}}
\newcommand{\directSumLimits}[1]{\underset{#1}{\mathlarger{\mathlarger{\oplus}}}}
\newcommand{\sampleSpaceGenCoord}{\mathcal D_{\redsolapproxST}}
\newcommand{\assLipschitz}{$(\bf{A}_1)$}
%\newcommand{\assInvLipschitz}{$(\bf{A}_3)$}
\newcommand{\assBounded}{$(\bf{A}_3)$}
\newcommand{\asssmallDt}{$(\bf{A}_2)$}
\newcommand{\asssmallDtNonlin}{$(\bf{A}_4)$}
\newcommand{\sigmamax}[1]{\sigma_\mathrm{max}(#1)}
\newcommand{\sigmamin}[1]{\sigma_\mathrm{min}(#1)}
\newcommand{\normEquiv}{P}
\newcommand{\lebesgue}{\Lambda}
\newcommand{\minimize}{\text{minimize}}



\newcounter{remctr}
\setcounter{remctr}{0}

\newcounter{propctr}
\setcounter{propctr}{0}
\newenvironment{property}{\refstepcounter{propctr}\begin{trivlist}
\item {\sc {Property \arabic{propctr}}.\:}}
{$\blacksquare$\end{trivlist}}

\newcounter{proposctr}
\setcounter{proposctr}{0}
\newenvironment{propos}{\refstepcounter{proposctr}\begin{trivlist}
\item {\sc {Proposition \arabic{proposctr}}.\:}}
{$\blacksquare $\end{trivlist}}
\newenvironment{proofofthing}[2]{\begin{trivlist}
\item {\sc {Proof of #1 \ref{#2}}.\:}}
{$\blacksquare $\end{trivlist}}


\newcommand{\RR}[1]{\ensuremath{\mathbb{R}^{ #1 }}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\RRplus}[1]{\ensuremath{\mathbb{R}_+^{ #1 }}}
\newcommand{\natNo}{\NN}
\newcommand{\nat}[1]{\natNo(#1)}
\newcommand{\natZero}[1]{\{0,\ldots,#1\}}
\newcommand{\innat}[1]{\in\nat{#1}}
\newcommand{\innatSeq}[1]{=1,\ldots,#1}
\newcommand{\innatZero}[1]{\in\natZero{#1}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\VV}{\mathbb{V}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\Image}[1]{\mathrm{Im}\left(#1\right)}
\newcommand{\Span}[1]{\mathrm{span}\{#1\}}
\newcommand{\Dim}[1]{\mathrm{dim}(#1)}
\newcommand{\vecmat}[2]{\bmat{#1^1 & \cdots& #1^{#2}}}
\newcommand{\entryvec}[3]{\left[#1_{#3_1} \ \cdots\ #1_{#3_{#2}}\right]^T}
\newcommand{\identity}[1]{\boldsymbol I_{#1}}
\newcommand{\nstepExtraction}{P_n}
\newcommand{\lipschitz}{\kappa}
\newcommand{\lipschitzst}{\bar{\lipschitz}}

\newcommand{\mass}{\Mbold}
\newcommand{\pexit}{P_\text{exit}}
\newcommand{\specificheat}{\gamma}
\newcommand{\energypermass}{\epsilon}
\newcommand{\densitySymb}{\rho}
\newcommand{\velocitySymb}{u}
\newcommand{\energydensity}{e}
\newcommand{\pressureSymb}{p}
\newcommand{\specificgasconstant}{R}
\newcommand{\speedofsoundSymb}{c}
\newcommand{\machSymb}{M}
\newcommand{\temperatureSymb}{T}
\newcommand{\resSymb}{r}
\newcommand{\resRedSymb}{{\mathsf r}}
\newcommand{\fluxSymb}{f}
\newcommand{\linearOperatorSymb}{L}
\newcommand{\paramSymb}{\mu}
\newcommand{\solSymb}{x}
\newcommand{\tensor}{\mathcal X}
\newcommand{\tensorUnfold}[1]{\boldsymbol{X}_{(#1)}}
\newcommand{\tensorReduceNo}{\mathcal X}
\newcommand{\tensorReduce}[1]{\tensorReduceNo(#1)}
\newcommand{\tensorresReduce}[1]{\tensorresReduceNo(#1)}
\newcommand{\tensorReduceUnfold}[2]{\boldsymbol{X}(#1)_{(#2)}}
\newcommand{\tensorres}{\mathcal R}
\newcommand{\tensorresUnfold}[1]{\boldsymbol{R}_{(#1)}}
\newcommand{\tensorresReduceNo}{\mathcal R}
\newcommand{\tensorresReduceUnfold}[2]{\boldsymbol{R}(#1)_{(#2)}}


\newcommand{\solFullDiscrete}{\mathbf{x}}
\newcommand{\solFullDiscreteOnlyParam}{\solFullDiscrete(\param)}
\newcommand{\solapproxFullDiscrete}{\tilde\mathbf{x}}
\newcommand{\solapproxFullDiscreteOnlyParam}{\tilde{\mathbf{x}}(\param)}
\newcommand{\solapproxSTFullDiscrete}{\tilde\mathbf{x}_\text{ST}}
\newcommand{\solapproxSTFullDiscreteOnlyParam}{\tilde{\mathbf{x}}_\text{ST}(\param)}
\newcommand{\unknownSymb}{w}
\newcommand{\spaceSymb}{s}
\newcommand{\timeSymb}{t}
\newcommand{\timestepit}{n}
\newcommand{\singvalmatSymb}{\Sigma}
\newcommand{\leftsingmatSymb}{U}
\newcommand{\rightsingmatSymb}{V}
\newcommand{\leftsingvecSymb}{u}
\newcommand{\rightsingvecSymb}{v}
\newcommand{\rearrangedrightsingvecspaceSymb}{K}
\newcommand{\weightmatSymb}{A}
\newcommand{\weightvecSymb}{a}
\newcommand{\basismatspaceSymb}{\Phi}
\newcommand{\basisvecspaceSymb}{\phi}
\newcommand{\basismattimeSymb}{\Psi}
\newcommand{\basisvectimeSymb}{\psi}
\newcommand{\basisvectimeFuncSymb}{\uppsi}
\newcommand{\basismatstSymb}{\Upsilon}
\newcommand{\basisvecstSymb}{\upsilon}
\newcommand{\operatorerroboundSymb}{\Xi}
\newcommand{\samplematSymb}{Z}
\newcommand{\samplevecSymb}{z}
\newcommand{\dummySymb}{y}
\newcommand{\snapshotSymb}{X}
\newcommand{\snapshotmatspaceSymb}{A}
\newcommand{\snapshotmattimeSymb}{B}
\newcommand{\stabilityconstantSymb}{h}


\newcommand{\nparam}{\smallnum_\mu}
\newcommand{\ntrain}{\smallnum_\text{train}}
\newcommand{\nparamROM}{\smallnum_{\hat\paramSymb}}
\newcommand{\nrestrain}{\smallnum_\text{res}}
\newcommand{\nressample}{\smallnum_{\samplevecSymb}}
\newcommand{\nressamplest}{\bar \smallnum_{\samplevecSymb}}
\newcommand{\nressamplestSmall}{\bar \smallnum_{\samplevecSymb}'}
\newcommand{\nrestimeind}{\bar \smallnum_{\timeSymb}}
\newcommand{\nresspaceind}{\bar \smallnum_{\spaceSymb}}
\newcommand{\nbasisres}{\smallnum_\resSymb}
\newcommand{\nbasisresst}{\bar \smallnum_\resSymb}
\newcommand{\nbasisspace}{{\smallnum_\spaceSymb}}
\newcommand{\nbasisspaceres}{{\smallnum_{\resSymb,\spaceSymb}}}
\newcommand{\nbasistime}{\smallnum_\timeSymb}
\newcommand{\nbasistimeres}{\smallnum_{\resSymb,\timeSymb}}
\newcommand{\nbasisst}{{\smallnum_{\spaceSymb\timeSymb}}}
\newcommand{\nbasisstTensor}{\sum_{i=1}^{\nbasisspace}\nbasistime^i}
\newcommand{\nspacedof}{\bignum_\spaceSymb}
\newcommand{\ntimedof}{{\bignum_\timeSymb}}
\newcommand{\nTimestepsFine}{\ntimedof}

\newcommand{\paramDomain}{\mathcal D}
\newcommand{\paramDomainTrain}{\paramDomain_\text{train}}
\newcommand{\paramDomainTrainres}{\paramDomain_\text{res}}
\newcommand{\ones}{\onebold}
\newcommand{\onesFunc}{\fontDiscreteFunc O}
\newcommand{\totaltime}{T}
\newcommand{\snapshotSubspace}{\fontDiscrete A}
\newcommand{\dimsnapshot}{r}
\newcommand{\spatialSubspace}{\fontDiscrete S}
\newcommand{\temporalSubspaceFunc}{\fontDiscreteFunc T}
\newcommand{\temporalSubspace}{\fontDiscrete T}
\newcommand{\spatiotemporalSubspaceFunc}{\fontDiscreteFunc{ST}}
\newcommand{\spatiotemporalSubspace}{\fontDiscrete{ST}}
\newcommand{\spacesampleset}{\mathfrak{s}}
\newcommand{\timesampleset}{\mathfrak{t}}
\newcommand{\PG}{\text{PG}}
\newcommand{\Tbe}{\boldsymbol A_\text{BE}}
\newcommand{\Alm}{\boldsymbol A_\text{LM}}
\newcommand{\Blm}{\boldsymbol B_\text{LM}}
\newcommand{\objective}{\zeta}
\newcommand{\operatorerrorboundSymb}{\Lambda}

\newcommand{\stabilityconstantBE}{\bar{\stabilityconstantSymb}_\text{be}}
\newcommand{\stabilityconstantLM}{\bar{\stabilityconstantSymb}_\text{lm}}
\newcommand{\tn}{\timeSymb^n}
\newcommand{\tnm}{\timeSymb^{n-1}}
\newcommand{\resSymbst}{\bar{\resSymb}}
\newcommand{\resRedSymbst}{\bar{\resRedSymb}}
\newcommand{\res}{\boldsymbol \resSymb}
\newcommand{\resk}{\boldsymbol \resSymb_k}
\newcommand{\reskn}{\boldsymbol \resSymb_{k(n)}}
\newcommand{\resArg}[1]{\boldsymbol \resSymb^{#1}}
\newcommand{\resRed}{\boldsymbol \resRedSymb}
\newcommand{\resRedApprox}{\tilde{\boldsymbol \resRedSymb}}
\newcommand{\resRedArg}[1]{\resRed(t^{#1})}
\newcommand{\resn}{\resArg{n}}
\newcommand{\resst}{\boldsymbol \resSymbst}
\newcommand{\resstApprox}{\tilde {\res}}
\newcommand{\resRedst}{\boldsymbol \resRedSymbst}
\newcommand{\resRedstapprox}{\bar{\tilde{\boldsymbol \resRedSymb}}}
\newcommand{\param}{\boldsymbol \paramSymb}
\newcommand{\paramTrain}[1]{\param^{#1}_\text{train}}
\newcommand{\paramTrainres}[1]{\param^{#1}_\text{res}}
\newcommand{\paramDummy}{\boldsymbol \nu}
\newcommand{\dt}{\Delta \timeSymb}
\newcommand{\dtArg}[1]{\dt^{#1}}
\newcommand{\sol}{\boldsymbol \solSymb}
\newcommand{\solw}{\boldsymbol w}
\newcommand{\solTimeContinuous}{\sol^\star}
\newcommand{\solst}{\bar{\sol}}
\newcommand{\solSymbst}{\bar{\solSymb}}
\newcommand{\flux}{\boldsymbol \fluxSymb}
\newcommand{\linearOp}{\boldsymbol \linearOperatorSymb}
\newcommand{\rhs}{\bar{\boldsymbol b}}
\newcommand{\rhsFunc}{\boldsymbol b}
\newcommand{\rhsFuncArg}[1]{\rhsFunc(t^{#1})}
\newcommand{\fluxst}{\bar{\flux}}
\newcommand{\solfom}{\sol_\star}
\newcommand{\solpgst}{\solst_{PG}}
\newcommand{\solfomst}{\solst_\star}
\newcommand{\solDummyScalar}{ w}
\newcommand{\solDummyScalarArg}[1]{\solDummyScalar^{#1}}
\newcommand{\solDummyScalarFuncArg}[1]{\solDummyScalar(t^{#1})}
\newcommand{\solDummy}{\boldsymbol w}
\newcommand{\solDummyst}{\bar\solDummy}
\newcommand{\solDummyArg}[1]{\solDummy^{#1}}
\newcommand{\solDummyFuncArg}[1]{\solDummy(t^{#1})}
\newcommand{\solDummyFuncArgDummy}[1]{\solDummy(\timeDummy^{#1})}
\newcommand{\solDummyOptFuncArg}[1]{\solDummyOpt(t^{#1})}
\newcommand{\solRedDummyScalar}{ \hat w}
\newcommand{\solRedDummyScalarArg}[1]{\solRedDummyScalar_{#1}}
\newcommand{\solRedDummy}{\hat {\boldsymbol w}}
\newcommand{\solDummyOpt}{{\boldsymbol \optDummy}}
\newcommand{\solRedDummyOpt}{\hat {\boldsymbol \optDummy}}
\newcommand{\timeArg}[1]{t^{#1}}
\newcommand{\timeDummy}{\tau}
\newcommand{\timeDomain}{[0,\totaltime]}
%\newcommand{\timestepset}{\mathfrak t}
\newcommand{\timestepset}{\{\timeArg{n}\}_{n=0}^{\ntimedof}}
\newcommand{\solFunc}{\sol}
\newcommand{\solinfty}{\sol_\infty}
\newcommand{\soltwo}{\sol_2}
\newcommand{\solFuncArg}[1]{\solFunc(t^{#1};\param)}
\newcommand{\solFuncOnlyParam}{\solFunc(\cdot;\param)}
\newcommand{\solFuncOnlyParamTrain}[1]{\solFunc(\cdot;\paramTrain{#1})}
\newcommand{\solFuncOnlyParamProject}{\hat\solFunc(\param)}
\newcommand{\solFuncOnlyParamProjectArg}[2]{\hat\solSymb_{#1#2}(\param)}
\newcommand{\solFuncn}{\solFuncArg{n}}
\newcommand{\solFuncnm}{\solFuncArg{n-1}}
%\newcommand{\solArg}[1]{\sol^{#1}(\param)}
\newcommand{\solArg}[1]{\sol(t^{#1};\param)}
\newcommand{\soln}{\solArg{n}}
\newcommand{\solnm}{\solArg{n-1}}
\newcommand{\spacetimesubspaceFunc}{\fontDiscreteFunc{ST}}
\newcommand{\spacetimesubspace}{\fontDiscrete{ST}}
\newcommand{\spacetimesubspacesmall}{\mathcal{ST}'}

\newcommand{\solapproxFunc}{\solapprox}
\newcommand{\solapproxFuncArg}[1]{\solapproxFunc(t^{#1};\param)}
\newcommand{\solapproxFuncArgs}[2]{\solapproxFunc_\text{#1}(t^{#2};\param)}
\newcommand{\solapproxFuncOnlyParam}{\solapproxFunc(\cdot;\param)}
\newcommand{\solapproxFuncn}{\solapproxFuncArg{n}}
\newcommand{\solapproxFuncnm}{\solapproxFuncArg{n-1}}

\newcommand{\redsolapproxFunc}{\redsolapprox}
\newcommand{\redsolapproxFuncArg}[1]{\redsolapproxFunc(t^{#1};\param)}
\newcommand{\redsolapproxFuncArgGen}[1]{\redsolapproxFunc(#1;\param)}
\newcommand{\redsolapproxFuncOnlyParam}{\redsolapproxFunc(\cdot;\param)}
\newcommand{\redsolapproxFuncn}{\redsolapproxFuncArg{n}}
\newcommand{\redsolapproxFuncnm}{\redsolapproxFuncArg{n-1}}

\newcommand{\redsolapproxEntryFunc}{\hat x}
\newcommand{\redsolapproxEntryFuncArg}[2]{\redsolapproxEntryFunc_{#1}(t^{#2};\param)}
\newcommand{\redsolapproxEntryFuncArgGen}[2]{\redsolapproxEntryFunc_{#1}(#2;\param)}
\newcommand{\redsolapproxEntryFuncOnlyParam}[1]{\redsolapproxEntryFunc_{#1}(\cdot;\param)}
\newcommand{\redsolapproxEntryFuncn}{\redsolapproxEntryFuncArg{n}}
\newcommand{\redsolapproxEntryFuncnm}{\redsolapproxEntryFuncArg{n-1}}




\newcommand{\penaltyparam}{\beta}
\newcommand{\lineSearchParam}{\alpha}
\newcommand{\lineSearchParamArg}[1]{\lineSearchParam^{(#1)}}
\newcommand{\testbasis}{\boldsymbol \Xi}
\newcommand{\testbasisArg}[2]{\boldsymbol \xi_{ij}}


\newcommand{\solapproxArg}[1]{\solapprox(t^{#1};\param)}
\newcommand{\solapproxArgs}[2]{\solapprox_\text{#1}(t^{#2};\param)}
\newcommand{\solapproxn}{\solapproxArg{n}}
\newcommand{\solapproxnm}{\solapproxArg{n-1}}

\newcommand{\redsolapproxArg}[1]{\redsolapprox(t^{#1};\param)}
\newcommand{\redsolapproxn}{\redsolapproxArg{n}}
\newcommand{\redsolapproxnm}{\redsolapproxArg{n-1}}

\newcommand{\paramTrainInitial}{\paramDomain_\text{initial}}
\newcommand{\paramTrainInitialArg}[1]{\param_\text{initial}^{#1}}
\newcommand{\nparamTrainInitial}{{n_{\paramSymb,\text{initial}}}}


\newcommand{\solSTscalar}{y}
\newcommand{\solST}{\boldsymbol{\solSTscalar}}
\newcommand{\solapproxSTFunc}{\tilde\solST}
\newcommand{\solapproxST}{\tilde\solST}
\newcommand{\solapproxSTFuncArg}[1]{\solapproxSTFunc(t^{#1};\param)}
\newcommand{\solapproxSTFuncArgs}[2]{\solapproxSTFunc_\text{#1}(t^{#2};\param)}
\newcommand{\solapproxSTFuncOnlyParam}{\solapproxSTFunc(\cdot;\param)}
\newcommand{\solapproxSTFuncn}{\solapproxSTFuncArg{n}}
\newcommand{\solapproxSTFuncnm}{\solapproxSTFuncArg{n-1}}
\newcommand{\solapproxSTArg}[1]{\solapproxSTFunc^{#1}(\param)}
\newcommand{\solapproxSTn}{\solapproxSTArg{n}}
\newcommand{\solapproxSTnm}{\solapproxSTArg{n-1}}

\newcommand{\redsolapproxST}{\hat\solST}
\newcommand{\redsolapproxSTVecArg}[1]{\redsolapproxST_{#1}(\param)}
\newcommand{\redsolapproxSTArg}[1]{\hat\solSTscalar_{#1}(\param)}
\newcommand{\redsolapproxSTArgNone}[1]{\hat\solSTscalar_{#1}}
\newcommand{\redsolapproxSTIt}[1]{\hat\solST^{(#1)}}
\newcommand{\deltaredsolapproxSTIt}[1]{\delta\hat\solST^{({#1})}}
\newcommand{\redsolapproxTrainNo}{\hat\solST_\text{res}}
\newcommand{\redsolapproxTrainArg}[1]{\redsolapproxTrainNo^{#1}}
\newcommand{\redsolapproxFOMTrainNo}{\hat\solST_\text{FOM}}
\newcommand{\redsolapproxFOMTrainArg}[1]{\redsolapproxFOMTrainNo(\paramTrain{#1})}
\newcommand{\redsolapproxFOMTrain}{\redsolapproxFOMTrainNo(\param)}
\newcommand{\stbasismat}{\boldsymbol \Pi}
\newcommand{\stbasisvec}[1]{\boldsymbol \pi_{#1}}
\newcommand{\stbasisvecFunc}[1]{\boldsymbol \uppi_{#1}}
\newcommand{\mseError}{\text{relative error}}



\newcommand{\solnfom}{\soln_\star}
\newcommand{\solnpg}{\sol_{PG}^n}
\newcommand{\solnmfom}{\sol_\star^{n-1}}
\newcommand{\solapprox}{\tilde\sol}
\newcommand{\redsolapprox}{\hat\sol}
\newcommand{\solapproxPG}{\solapprox_\PG}
\newcommand{\redsol}{\hat\sol}
\newcommand{\redsoln}{\redsol^n}
\newcommand{\redsolst}{\redsol}
\newcommand{\redsolstSol}{\redsol_\star}
\newcommand{\redsolstij}[2]{\hat\solSymb_{#1#2}}
\newcommand{\soli}[1]{\sol^{#1}}
\newcommand{\solEntry}[1]{\solSymb_{#1}}
\newcommand{\resEntryi}[1]{\mathsf\resSymb_{#1}}
\newcommand{\unknown}{\boldsymbol{\unknownSymb}}
\newcommand{\unknowni}[1]{\unknown_{#1}}
\newcommand{\dummy}{\boldsymbol {\dummySymb}}
\newcommand{\reddummy}{\hat{\dummy}}
\newcommand{\reddummyij}[2]{\hat{\dummySymb}_{#1#2}}
\newcommand{\redres}{\hat{\res}}
\newcommand{\solinit}{\sol^0}
\newcommand{\solinitEntry}[1]{\solSymb_{#1}^0}
\newcommand{\solinitst}{\bar{\sol}^0}
%\newcommand{\solref}{\sol_{\text{ref}}}
\newcommand{\solref}{\solinit(\param)}
\newcommand{\solrefst}{\bar{\sol}_{\text{ref}}}
\newcommand{\singvalmat}{\boldsymbol \singvalmatSymb}
\newcommand{\singvalmatspace}{\singvalmat_\spaceSymb}
\newcommand{\singvalmatspaceres}{\singvalmat_{\resSymb,\spaceSymb}}
\newcommand{\singvalmattime}{\singvalmat_\timeSymb}
\newcommand{\singvalmattimeres}{\singvalmat_{\resSymb,\timeSymb}}
\newcommand{\leftsingvec}{\boldsymbol{\leftsingvecSymb}}
\newcommand{\rightsingvec}{\boldsymbol{\rightsingvecSymb}}
\newcommand{\leftsingvecspace}{\leftsingvec_\spaceSymb}
\newcommand{\leftsingvecspaceres}{\leftsingvec_{\resSymb,\spaceSymb}}
\newcommand{\leftsingvectime}{\leftsingvec_\timeSymb}
\newcommand{\leftsingvectimeres}{\leftsingvec_{\resSymb,\timeSymb}}
\newcommand{\leftsingvectimeArg}[1]{\leftsingvectime^{#1}}
\newcommand{\leftsingvectimeresArg}[1]{\leftsingvectimeres^{#1}}
\newcommand{\rightsingvecspace}{\rightsingvec_\spaceSymb}
\newcommand{\rightsingvectime}{\rightsingvec_\timeSymb}
\newcommand{\leftsingvecspacei}[1]{\leftsingvecspace^{#1}}
\newcommand{\leftsingvecspaceresi}[1]{\leftsingvecspaceres^{#1}}
\newcommand{\leftsingvectimei}[1]{\leftsingvectime^{#1}}
\newcommand{\leftsingvectimeij}[2]{\leftsingvectime^{#1,#2}}
\newcommand{\rightsingvecspacei}[1]{\rightsingvecspace^{#1}}
\newcommand{\rightsingvecspaceij}[2]{\rightsingvec_{\spaceSymb,#2}^{#1}}
\newcommand{\rightsingvectimei}[1]{\rightsingvectime^{#1}}
\newcommand{\rightsingvecspaceSymbij}[2]{\rightsingvecSymb_{\spaceSymb,#1}^{#2}}
\newcommand{\leftsingmat}{\boldsymbol{\leftsingmatSymb}}
\newcommand{\rightsingmat}{\boldsymbol{\rightsingmatSymb}}
\newcommand{\leftsingmatspace}{\leftsingmat_\spaceSymb}
\newcommand{\leftsingmatspaceres}{\leftsingmat_{\resSymb,\spaceSymb}}
\newcommand{\leftsingmattime}{\leftsingmat_\timeSymb}
\newcommand{\leftsingmattimei}[1]{\leftsingmattime^{#1}}
\newcommand{\leftsingmattimeres}{\leftsingmat_{\resSymb,\timeSymb}}
\newcommand{\leftsingmattimeresi}[1]{\leftsingmattimeres^{#1}}
\newcommand{\rightsingmatspace}{\rightsingmat_\spaceSymb}
\newcommand{\rightsingmatspaceres}{\rightsingmat_{\resSymb,\spaceSymb}}
\newcommand{\rightsingmattime}{\rightsingmat_\timeSymb}
\newcommand{\rightsingmattimeres}{\rightsingmat_{\resSymb,\timeSymb}}
\newcommand{\rightsingmattimei}[1]{\rightsingmattime^{#1}}
\newcommand{\rearrangedrightsingvecspace}{\boldsymbol \rearrangedrightsingvecspaceSymb}
\newcommand{\rearrangedrightsingvecspacei}[1]{\rearrangedrightsingvecspace^{#1}}
\newcommand{\basismattime}{\boldsymbol{\basismattimeSymb}}
\newcommand{\basismattimei}[1]{\basismattime^{#1}}
\newcommand{\basisvectime}{\boldsymbol{\basisvectimeSymb}}
\newcommand{\basisvectimei}[1]{\basisvectime_{#1}}
\newcommand{\basisvectimeij}[2]{\basisvectime^{#1}_{#2}}
\newcommand{\basisvectimeijk}[3]{{\basisvectimeSymb}^{#1}_{#2#3}}
\newcommand{\basisvectimeresi}[1]{\basisvectime_{r,#1}}
\newcommand{\basisvectimeresij}[2]{\basisvectime^{#1}_{r,#2}}
\newcommand{\basisvectimeresijk}[3]{{\basisvectimeSymb}^{#1}_{r,#2#3}}
\newcommand{\basisvectimeFunc}{\boldsymbol{\basisvectimeFuncSymb}}
\newcommand{\basisvectimeFuncij}[2]{\basisvectimeFunc_{#2}^{#1}}
\newcommand{\basisvectimeresFuncij}[2]{\basisvectimeFunc_{r,#2}^{#1}}
\newcommand{\basisvectimeFunci}[1]{\basisvectimeFunc_{#1}}
\newcommand{\basisvectimeresFunci}[1]{\basisvectimeFunc_{r,#1}}
\newcommand{\basisvectimeFuncVeci}[1]{\basisvectimeFunc^{#1}}
\newcommand{\basisvectimeFuncijk}[3]{{\basisvectimeFuncSymb}^{#1}_{#2#3}}
\newcommand{\basisvecFunctime}{\boldsymbol{\basisvectimeFuncSymb}}
\newcommand{\basisvecFunctimeij}[2]{\basisvectimeFunc^{#1}_{#2}}
\newcommand{\basisvecFunctimeijk}[3]{{\basisvectimeFuncSymb}^{#1}_{#2#3}}
\newcommand{\basismatst}{\boldsymbol{\basismatstSymb}}
\newcommand{\basisvecst}{\boldsymbol{\basisvecstSymb}}
\newcommand{\operatorerrorbound}{\boldsymbol{\operatorerrorboundSymb}}
\newcommand{\basisDummy}{\boldsymbol{V}}
\newcommand{\basismatspace}{\boldsymbol{\basismatspaceSymb}}
\newcommand{\basismatspaceres}{\boldsymbol{\basismatspaceSymb}_r}
\newcommand{\basisvecspace}{\boldsymbol{\basisvecspaceSymb}}
\newcommand{\basisvecspaceres}{\boldsymbol{\basisvecspaceSymb}_r}
\newcommand{\basisvecspacei}[1]{\boldsymbol{\basisvecspaceSymb}_{#1}}
\newcommand{\basisvecspaceresi}[1]{\boldsymbol{\basisvecspaceSymb}_{r,#1}}
\newcommand{\basismatres}{\basismatspace_\resSymb}
\newcommand{\basismatrest}{{\bar \basismatspace}_\resSymb}
\newcommand{\basismatrestvec}[1]{{\bar {\boldsymbol{\basisvecspaceSymb}}_{r,#1}}}
\newcommand{\basismatrestvecFunc}[1]{{\bar
{\boldsymbol{\upphi}}_{r,#1}}}
\newcommand{\basisresi}[1]{\basismatrest^{#1}}
\newcommand{\basisres}{\boldsymbol \Pi_r}
\newcommand{\mappingresNo}{\mathcal I_r}
\newcommand{\mappingres}[2]{\mappingresNo(#1,#2)}
\newcommand{\basisresvecArg}[1]{\boldsymbol \pi_{r,#1}}
\newcommand{\basisresvecij}[2]{\basisresvecArg{\mappingres{#1}{#2}}}
\newcommand{\rfactor}{{\boldsymbol R}}
\newcommand{\basisvecres}{\basisvecspace_{\resSymb}}
\newcommand{\basisvecresst}{\bar{\basisvecspace}_{\resSymb}}
\newcommand{\basisvecressti}[1]{\basismatrestvec{#1}}
\newcommand{\basisvecresstij}[2]{\bar \basisvecspaceSymb_{\resSymb({#1},{#2})}}
\newcommand{\errorvec}{\boldsymbol \varepsilon}
\newcommand{\errorvecFunc}{\boldsymbol \upvarepsilon}
\newcommand{\errorvecFuncEntry}[1]{\upvarepsilon_{#1}}
\newcommand{\timesamplestoadd}[1]{\nrestimeind^{#1}}
\newcommand{\spacesamplestoadd}[1]{\nresspaceind^{#1}}
\newcommand{\spacetimesamplestoadd}[1]{\nressamplest^{#1}}
\newcommand{\minsamplestoadd}{\bar n_{\timeSymb,\text{min}}}
\newcommand{\weightmat}{\boldsymbol{\weightmatSymb}}
\newcommand{\weightmatst}{\bar\weightmat}
\newcommand{\weightmatstArg}[1]{\weightmatst^{#1}}
\newcommand{\weightvecstij}[2]{\bar{\weightvecSymb}_{{#1}{#2}}}
\newcommand{\snapshots}{\boldsymbol \snapshotSymb}
\newcommand{\snapshotsRes}{\boldsymbol R}
%\newcommand{\snapshotmatspace}{\boldsymbol \snapshotmatspaceSymb}
%\newcommand{\snapshotmattime}{\boldsymbol \snapshotmattimeSymb}
\newcommand{\snapshotmatspace}{\tensorUnfold{1}}
\newcommand{\snapshotmattime}{\tensorUnfold{2}}

%\newcommand{\resn}{\res^{n}}
\newcommand{\resnst}{\resst^{n}}
\newcommand{\samplemat}{\boldsymbol \samplematSymb}
\newcommand{\samplematst}{\bar{\samplemat}}
\newcommand{\samplevec}{\boldsymbol \samplevecSymb}
\newcommand{\samplevecst}{\bar{\samplevec}}
\newcommand{\samplevecsti}[1]{\samplevecst_{#1}}
\newcommand{\resi}[1]{\res^{{#1}}}
\newcommand{\snapshotSubspacei}[1]{\snapshotSubspace_{#1}}
\newcommand{\spatialSubspacei}[1]{\spatialSubspace_{#1}}
\newcommand{\temporalSubspaceFuncArg}[1]{\temporalSubspaceFunc_{#1}}
\newcommand{\temporalSubspaceArg}[1]{\temporalSubspace_{#1}}



\newcommand{\bmat}[1]{\begin{bmatrix}#1\end{bmatrix}} % Need \usepackage{amsmath}
\newcommand{\pmat}[1]{\begin{pmatrix}#1\end{pmatrix}} % Need \usepackage{amsmath}
\newcommand{\vmat}[1]{\begin{vmatrix}#1\end{vmatrix}} % Need \usepackage{amsmath}
\newcommand{\Vmat}[1]{\begin{Vmatrix}#1\end{Vmatrix}} % Need \usepackage{amsmath}
\newcommand{\Bmat}[1]{\begin{Bmatrix}#1\end{Bmatrix}} % Need \usepackage{amsmath}
\newcommand{\blue}{\textcolor{blue}}
\newcommand{\red}{\textcolor{red}}
\newcommand{\yellow}{\textcolor{yellow}}
\newcommand{\cyan}{\textcolor{cyan}}
\newcommand{\green}{\textcolor{green}}
\def\Abb{\mathbb{A}}
\def\Bbb{\mathbb{B}}
\def\Cbb{\mathbb{C}}
\def\Dbb{\mathbb{D}}
\def\Ebb{\mathbb{E}}
\def\Fbb{\mathbb{F}}
\def\Gbb{\mathbb{G}}
\def\Hbb{\mathbb{H}}
\def\Ibb{\mathbb{I}}
\def\Jbb{\mathbb{J}}
\def\Kbb{\mathbb{K}}
\def\Lbb{\mathbb{L}}
\def\Mbb{\mathbb{M}}
\def\Nbb{\mathbb{N}}
\def\Obb{\mathbb{O}}
\def\Pbb{\mathbb{P}}
\def\Qbb{\mathbb{Q}}
\def\Rbb{\mathbb{R}}
\def\Sbb{\mathbb{S}}
\def\Tbb{\mathbb{T}}
\def\Ubb{\mathbb{U}}
\def\Vbb{\mathbb{V}}
\def\Wbb{\mathbb{W}}
\def\Xbb{\mathbb{X}}
\def\Ybb{\mathbb{Y}}
\def\Zbb{\mathbb{Z}}
\def\onebold{\boldsymbol{1}}
\def\Abold{\boldsymbol{A}}
\def\Bbold{\boldsymbol{B}}
\def\Cbold{\boldsymbol{C}}
\def\Dbold{\boldsymbol{D}}
\def\Ebold{\boldsymbol{E}}
\def\Fbold{\boldsymbol{F}}
\def\Gbold{\boldsymbol{G}}
\def\Hbold{\boldsymbol{H}}
\def\Ibold{\boldsymbol{I}}
\def\Jbold{\boldsymbol{J}}
\def\Kbold{\boldsymbol{K}}
\def\Lbold{\boldsymbol{L}}
\def\Mbold{\boldsymbol{M}}
\def\Nbold{\boldsymbol{N}}
\def\Obold{\boldsymbol{O}}
\def\Pbold{\boldsymbol{P}}
\def\Qbold{\boldsymbol{Q}}
\def\Rbold{\boldsymbol{R}}
\def\Sbold{\boldsymbol{S}}
\def\Tbold{\boldsymbol{T}}
\def\Ubold{\boldsymbol{U}}
\def\Vbold{\boldsymbol{V}}
\def\Wbold{\boldsymbol{W}}
\def\Xbold{\boldsymbol{X}}
\def\Ybold{\boldsymbol{Y}}
\def\Zbold{\boldsymbol{Z}}
\def\abold{\boldsymbol{a}}
\def\bbold{\boldsymbol{b}}
\def\cbold{\boldsymbol{c}}
\def\dbold{\boldsymbol{d}}
\def\ebold{\boldsymbol{e}}
\def\fbold{\boldsymbol{f}}
\def\gbold{\boldsymbol{g}}
\def\hbold{\boldsymbol{h}}
\def\ibold{\boldsymbol{i}}
\def\kbold{\boldsymbol{k}}
\def\qbold{\boldsymbol{q}}
\def\pbold{\boldsymbol{p}}
\def\rbold{\boldsymbol{r}}
\def\sbold{\boldsymbol{s}}
\def\tbold{\boldsymbol{t}}
\def\ubold{\boldsymbol{u}}
\def\vbold{\boldsymbol{v}}
\def\wbold{\boldsymbol{w}}
\def\xbold{\boldsymbol{x}}
\def\ybold{\boldsymbol{y}}
\def\zbold{\boldsymbol{z}}
\def\alphabold{\boldsymbol{\alpha}}
\def\lambdabold{\boldsymbol{\lambda}}
\def\betabold{\boldsymbol{\beta}}
\def\etabold{\boldsymbol{\eta}}
\def\gammabold{\boldsymbol{\gamma}}
\def\deltabold{\boldsymbol{\delta}}
\def\mubold{\boldsymbol{\mu}}
\def\phibold{\boldsymbol{\phi}}
\def\psibold{\boldsymbol{\psi}}
\def\Phibold{\boldsymbol{\Phi}}
\def\Sigmabold{\boldsymbol{\Sigma}}
\def\sigmabold{\boldsymbol{\sigma}}
\def\Gammabold{\boldsymbol{\Gamma}}
\def\Omegabold{\boldsymbol{\Omega}}
\def\Thetabold{\boldsymbol{\Theta}}
\def\Lambdabold{\boldsymbol{\Lambda}}
\def\Psibold{\boldsymbol{\Psi}}
\def\xibold{\boldsymbol{\xi}}
\def\zetabold{\boldsymbol{\zeta}}
\def\zerobold{{\bf 0}}
\def\ds{\displaystyle} 
\def\enorm#1{\|#1\|_2} 
\def\norm#1{\|#1\|} 
\def\fortran{{FORTRAN}} 
\def\gmres{{GMRES}} 
\def\bfE{\mbox{\boldmath$E$}}
\def\bfG{\mbox{\boldmath$G$}}

%Karen Added
\newcommand{\jjprime}{(j,j^\prime)}

\newcommand{\Amatrix}{\constraintMatROM(\mubold) }
\newcommand{\Bhatmatrix}{\bds{B}(\mubold) }
\newcommand{\uinit}{\bds{u}_{0}(\mubold) }

\newcommand{\AhatPetrovGalerkin}{\hat{\constraintMatROM}^{st, pg}(\mubold) }
\newcommand{\AhatPetrovGalerkinBlock}{\hat{\constraintMatROM}^{st, pg}_{\jjprime}(\mubold) }
\newcommand{\temporalBasisMatrixk}{\bds{D}_k}
\newcommand{\temporalBasisMatrixkpone}{\bds{D}_{k+1}}
\newcommand{\fhatPetrovGalerkin}{\hat{\bds{f}}^{st, pg}}
\newcommand{\fhatGalerkin}{\hat{\bds{f}}^{st}}
\newcommand{\uhatPetrovGalerkin}{\hat{\bds{u}_0}^{st, pg}}
\newcommand{\uhatGalerkin}{\hat{\bds{u}_0}^{st}}


\newcommand{\IdentityNs}{\bds{I}_{N_s}}



\newcommand{\AhatGalerkin}{\hat{\constraintMatROM}^{st}(\mubold) }

\newcommand{\Astparameter}{\constraintMatROM^{st} (\mubold)   }


==> packages.tex <==
%\usepackage{fullpage}
\usepackage{upgreek}
\usepackage{mathdots}
\usepackage{BOONDOX-calo}
\usepackage[mathscr]{eucal}
\usepackage{color}
\usepackage[usenames,dvipsnames,svgnames,table]{xcolor}
\usepackage{amsmath,amssymb,amsopn,mathtools}
\usepackage{graphicx}
%\usepackage{algorithmic}
%\usepackage{algorithm}
%\usepackage{geometry}
%\usepackage{wasysym}
%\usepackage{url}
%\usepackage{float}
%\usepackage[makeroom]{cancel}
%\usepackage{marginnote}
%\usepackage{sfmath} 

\usepackage{hyperref}       % internal hyperlink to contents
\hypersetup{
	colorlinks=true,   % boxed links
	%    colorlinks=false,   % colored links
	citecolor=blue,     % citation links (bibliography)
	filecolor=blue,     % color of file links
	linkcolor=red,    % internal links (sections, pages, etc.)
	urlcolor=blue}      % color of URL links (mail, web)

%\usepackage{atbegshi}% http://ctan.org/pkg/atbegshi
%
%\AtBeginDocument{\AtBeginShipoutNext{\AtBeginShipoutDiscard}}
\usepackage{relsize}
%\usepackage{amsthm}
\numberwithin{equation}{section}

